UniCoN: Universal Conditional Networks for Multi-Age Embryonic Cartilage Segmentation with Sparsely Annotated Data

Osteochondrodysplasia, affecting 2-3% of newborns globally, is a group of bone and cartilage disorders that often result in head malformations, contributing to childhood morbidity and reduced quality of life. Current research on this disease using mouse models faces challenges since it involves accurately segmenting the developing cartilage in 3D micro-CT images of embryonic mice. Tackling this segmentation task with deep learning (DL) methods is laborious due to the big burden of manual image annotation, expensive due to the high acquisition costs of 3D micro-CT images, and difficult due to embryonic cartilage's complex and rapidly changing shapes. While DL approaches have been proposed to automate cartilage segmentation, most such models have limited accuracy and generalizability, especially across data from different embryonic age groups. To address these limitations, we propose novel DL methods that can be adopted by any DL architectures -- including CNNs, Transformers, or hybrid models -- which effectively leverage age and spatial information to enhance model performance. Specifically, we propose two new mechanisms, one conditioned on discrete age categories and the other on continuous image crop locations, to enable an accurate representation of cartilage shape changes across ages and local shape details throughout the cranial region. Extensive experiments on multi-age cartilage segmentation datasets show significant and consistent performance improvements when integrating our conditional modules into popular DL segmentation architectures. On average, we achieve a 1.7% Dice score increase with minimal computational overhead and a 7.5% improvement on unseen data. These results highlight the potential of our approach for developing robust, universal models capable of handling diverse datasets with limited annotated data, a key challenge in DL-based medical image analysis.

==> new_sections/postReferencesSection.tex <==
\vspace{-3.5mm}
\section*{Author Contributions}
\vspace{-1mm}
KK, GH, MW, and EWJ supplied the mice. SMMP, YH, and JAW acquired the data. NS, YZ, and DZC designed the method and experiments. NS conducted the experiments with the help of ZZ and MG. NS, YZ, JAW, SMMP, and DZC wrote the manuscript. All the authors reviewed the manuscript.
\vspace{-2mm}
\section*{Additional Information}
\vspace{-1mm}
The authors declare that there are no conflicts of interest regarding this publication.
\vspace{-2mm}
\section*{Acknowledgements}
\vspace{-1mm}
This research was supported in part by NIH NIDCR grants R01 DE031439 (awarded to SMMP, EWJ, and KK) and R01 DE029832 (awarded to EWJ, KK, and SMMP) and the CSE Select Fellowship of the Graduate School at the University of Notre Dame (for NS). We extend our appreciation to The Pennsylvania State University Center for Quantitative Imaging for providing high-quality images, and to the research technicians for their invaluable assistance in the preparation of the samples.
% \section*{Additional Information}
% \notes{To include, in this order: \textbf{Accession codes} (where applicable); \textbf{Competing interests} (mandatory statement).  The corresponding author is responsible for submitting a competing interests statement on behalf of all authors of the paper. This statement must be included in the submitted article file.}
% \href{http://www.nature.com/srep/policies/index.html#competing}{Acess Here}
